Time-integration of Gaussian variational approximation for the magnetic Schr\"odinger equation

In the present paper we consider the semiclassical magnetic Schr\"odinger equation, which describes the dynamics of charged particles under the influence of a electro-magnetic field. The solution of the time-dependent Schr\"odinger equation is approximated by a single Gaussian wave packet via the time-dependent Dirac--Frenkel variational principle. For the approximation we use ordinary differential equations of motion for the parameters of the variational solution and extend the second-order Boris algorithm for classical mechanics to the quantum mechanical case. In addition, we propose a modified version of the classical fourth order Runge--Kutta method. Numerical experiments explore parameter convergence and geometric properties. Moreover, we benchmark against the analytical solution of the Penning trap.

==> old-stuff/EffectivePotential.tex <==
The two approximations differ, in particular, with respect to their effective electric potential, which in both cases is a polynomial of degree $\le 2$, but with different coefficients. For notational simplicity, we consider the case of a time-independent potential $\phi(x)$ in the following, without loss of generality. 

\subsubsection{Classical approximation} 
The classical effective potential is the second order Taylor polynomial of~$\mltPot$ expanded around the center point $\pos_t$ of the approximate Gaussian,
\begin{equation}\label{eq:poteff_cl}
\mltPot_{\rm eff}^{\rm cl}(t,x) = \mltPot(\pos_t) + \nabla \mltPot(\pos_t)^\top (x-\pos_t) + 
\frac12 (x-\pos_t)^\top \nabla^2 \mltPot(\pos_t) (x-\pos_t).
\end{equation}
Comparing the original potential $\mltPot(x)$ and the effective $\mltPot_{\rm eff}^{\rm cl}(t,x)$, there is just the remainder of the second order Taylor approximation, which can be bounded by a cubic polynomial in $x-\pos_t$.

\subsubsection{Variational approximation}
The variational effective potential is a polynomial of degree two as well, but has averaged coefficients, 
\begin{equation}\label{eq:poteff_va}
\mltPot_{\rm eff}^{\rm va}(t,x) = \alpha_0(t) + a_1(t)^\top (x-\pos_t) + 
\frac12 (x-\pos_t)^\top A_2(t) (x-\pos_t)
\end{equation}
with
\begin{align}
\alpha_0(t) &= \langle \mltPot\rangle_{\vsol} - \frac\scp4 \tr\!\left(\ICinv\langle \nabla^2 \mltPot\rangle_{\vsol} \right) = \mltPot(\pos_t) + \mathcal O(\scp^2),\\*[1ex] 
a_1(t) &= \langle \nabla \mltPot\rangle_{\vsol}
= \nabla \mltPot(\pos_t) + \frac\scp4 \tr\!\left(\ICinv \nabla^2 \partial_j \mltPot(\pos_t)\right)_{j=1}^\dim + \mathcal O(\scp^2),\\*[1ex] 
A_2(t) &= \langle \nabla^2 \mltPot\rangle_{\vsol}
=\nabla^2 \mltPot(\pos_t) + \mathcal O(\scp),
\end{align}
see \cite[Proposition 3.14]{LasL20} for the effective potential and \cite[Proposition 7.4]{BurDHL24} for the expansion of the averages. Its coefficients differ from the one of the classical Taylor polynomial on the order of $\scp$ and $\scp^2$. 

\subsubsection{Comparison of the effective potentials}
We next analyze the two effective potentials $\mltPot_{\rm eff}$ with respect to the key quantities that build up the error estimates in \eqref{eq:error_all}. For the norm estimate \eqref{eq:error_norm}, the effective potential contributes via the integral
\[
\frac1\scp\int_0^t \normLtwo{\left(\mltPot-\mltPot_{\rm eff}(s)\right) \vsol(s)} \mathrm{d}s,
\]
see the proof of \cite[Theorem 3.8]{BurDHL24}. Here, the classical and the variational approximation only differ in the error constant. For the observable error \eqref{eq:error_obs}, it is the representation formula \cite[Lemma~7.1]{BurDHL24}, which contains a commutator-like expression, such that the effective potential contributes via an average of the form
\[
\int_0^t \left\langle a\,\partial_x\left(\mltPot-\mltPot_{\rm eff}(s)\right)\right\rangle_{\vsol(s)}\mathrm{d}s,
\]
where $a$ is function related to the time propagation of the observable $\obs$. For the observable error, the variational convergence order is higher than the classical one. For the ease of presentation, but without loss of generality, we restrict ourselves to dimension $d=1$ in the following, where we extend the key elements of the error analysis given in \cite{BurDHL24} to the point that the crucial parts of the error constants become explicit, in particular the dependence on the width of the Gaussian wave packet.

\begin{prop} Consider a uni-variate classical or variational normalized \GWP $\vsol(t)\in\Mf$ with center $\pos_t$ and width parameter $\wm_t = \IC(t)+\ii\RC(t)$. Then, the effective potentials $\mltPot_{\rm eff}(t)$ defined in \eqref{eq:poteff_cl} or \eqref{eq:poteff_va}, respectively, satisfy the following estimates.
\begin{enumerate}
\item Norm difference:
\[
\normLtwo{\left(\mltPot-\mltPot_{\rm eff}(t)\right) \vsol(t)} =  c_{\rm eff}\, \mltPot'''(q_t)\, \IC(t)^{-3/2} \scp^{3/2} + \mathcal O(\scp^2)
\]
with constants $c_{\rm eff}>0$ given as 
\[
c_{\rm eff} = \left\{\begin{array}{lc} \sqrt{30}/24 \approx 0.23 & \text{(classical)}\\*[1ex]
\sqrt{3}/12\approx 0.14 & \text{(variational)}\end{array}\right.
\]
\item Averaged derivative difference: For any smooth function $a:\bbR\to\bbR$,
\[
\left\langle a\,\partial_x\left(\mltPot-\mltPot_{\rm eff}(t)\right)\right\rangle_{\vsol(t)} = 
\left\{\begin{array}{lc}
\frac14 a(\pos_t)\,\mltPot'''(\pos_t)\, \IC(t)^{-1}\scp + \mathcal O(\scp^2) & \text{(class.)}\\*[1ex]
\frac{1}{8} a''(\pos_t)\,\mltPot'''(\pos_t) \,\IC(t)^{-2}\scp^2 + \mathcal O(\scp^3) & \text{(var.)}
\end{array}\right.
\] 
\end{enumerate}
\end{prop}

\begin{proof}
(a) We start by analyzing the difference in norm. 
Note that the normalization of $\vsol$ implies
\begin{equation}
 1 = \normLtwo{\vsol}^2 
 =  \int_{-\infty}^\infty  \exp\!\left(-\frac{\IC(t)}{\scp}x^2 - \frac{2}{\scp}\ImPha(t)\right) \dx
 =\sqrt{\pi} \e^{- \frac{2}{\scp}\ImPha(t)}  \Bigl( \frac{\scp}{\IC(t)} \Bigr)^{1/2}.
\end{equation}
Hence, the even moments are given by
\begin{equation}  \label{eq:moments}
    \mean{(x-\pos_t)^{2m}} =  \frac{(2m-1)!!}{2^m} \Bigl( \frac{\scp}{\IC(t)} \Bigr)^{m},
\end{equation}
while the odd moments vanish. In particular, this implies that a polynomial $(x-\pos_t)^m$ times $\vsol$ is of the order $\scp^{m/2}$ in $L^2(\bbR)$, see also \cite[Lemma 3.8]{LasL20}. Therefore, we have
\begin{align}
&\left(\mltPot(x)-\mltPot_{\rm eff}^{\rm cl}(t,x)\right) u(t,x) 
= \frac16 \mltPot'''(\pos_t)\, (x-\pos_t)^3 u(t,x) + \mathcal O(\scp^2),
\end{align}
and we obtain the square of the norm of the leading function as
\begin{align}
\frac{1}{36} \normLtwo{(x-\pos_t)^3 \vsol(t)}^2 = \frac{5\scp^3 }{96\, \IC(t)^3}.
\end{align}
% \textcolor{red}{MH with
% \begin{equation}
% \int_{-\infty}^\infty x^{2m} \e^{-ax^2} \dx = \frac{\sqrt{\pi} (2m-1)!!}{2^m a^{(2m+1)/2}}
% \end{equation}
% I get
% \begin{align}
% \frac{1}{36}\int_{-\infty}^\infty  (x-\pos_t)^6 \left|u(t,x)\right|^2 \dx 
% &=\frac{1}{36} \int_{-\infty}^\infty  x^6\ \e^{-\frac{\IC(t)}{\scp}x^2 - \frac{2}{\scp}\ImPha(t)} \dx\\
% &=\frac{5 {\sqrt{\pi} }}{12\cdot 8} \e^{- \frac{2}{\scp}\ImPha(t)}  \frac{\scp^{7/2}}{\IC(t)^{7/2}}\\
% & \textcolor{blue}{
% = \frac{5 }{12\cdot 8} \frac{\scp^{3}}{\IC(t)^{3}}}
% \end{align}
% }
Turning to the variational potential, we use 
the asymptotic expansion of its coefficients $\alpha_0(t), a_1(t), A_2(t)$ with respect to $\scp$ and obtain
\begin{align}
&\left(\mltPot(x)-\mltPot_{\rm eff}^{\rm va}(t,x)\right) u(t,x) \\
&= \mltPot'''(\pos_t)\, (x-\pos_t)
\left(-\frac\scp4\ICinv(t) + \frac16 (x-\pos_t)^2\right)u(t,x) + \mathcal O(\scp^2).
\end{align}
Using \eqref{eq:moments}, we have
\begin{align}
&\int_{-\infty}^\infty (x-\pos_t)^2 
\left(
    -\frac\scp4\ICinv(t) + \frac16 (x-\pos_t)^2
\right)^2 |u(t,x)|^2 \dx \\
&= 
\frac{1}{16} \mean{(x-\pos_t)^2} \Bigl( \frac{\scp}{\IC(t)} \Bigr)^{2}
-
\frac{1}{12} \mean{(x-\pos_t)^4} \Bigl( \frac{\scp}{\IC(t)} \Bigr)
+
\frac{1}{36} \mean{(x-\pos_t)^6} \\
&= 
\frac{1}{48} \Bigl( \frac{\scp}{\IC(t)} \Bigr)^{3}.
% \Bigl( \frac{\scp}{\IC(t)} \Bigr)^{3}
% &= \e^{- \frac{2}{\scp}\ImPha(t)} \int_{-\infty}^\infty x^2 
% \left(-\tfrac\scp4\ICinv(t) + \tfrac16 x^2\right)^2  \e^{-\frac{\IC(t)}{\scp} x^2} \dx \\
% &= \frac{\sqrt{\pi}}{48} \e^{- \frac{2}{\scp}\ImPha(t)} \frac{\scp^{7/2}}{\IC(t)^{7/2}}\\
% & \textcolor{blue}{=\frac{\scp^3}{48 \IC(t)^3}} 
\end{align}

(b) We next turn to the averaged derivative difference. By Taylor expansion, we have
\begin{align}
&\partial_x\left(\mltPot(x)-\mltPot^{\rm cl}_{\rm eff}(t,x)\right) =\\ 
&\frac12 \mltPot'''(\pos_t) (x-\pos_t)^2 + \frac16 \mltPot^{(4)}(\pos_t)(x-\pos_t)^3 + 
\mathcal O((x-\pos_t)^4)
\end{align}
and
\begin{align}
&a(x)\,\partial_x\left(\mltPot(x)-\mltPot^{\rm cl}_{\rm eff}(t,x)\right) = 
\frac12 a(\pos_t) \mltPot'''(\pos_t) (x-\pos_t)^2 \\
&+ \left(\frac16 a(\pos_t)\mltPot^{(4)}(\pos_t) + \frac12 a'(q_t)\mltPot'''(\pos_t)\right)(x-\pos_t)^3 + 
\mathcal O((x-\pos_t)^4).
\end{align}
Therefore, again by \eqref{eq:moments},
\begin{align}
\left\langle a\,\partial_x(\mltPot-\mltPot_{\rm eff}^{\rm cl}(t))\right\rangle_{\vsol(t)} 
&= 
 \frac12 a(\pos_t)\,\mltPot'''(\pos_t) \langle (x-\pos_t)^2\rangle_{\vsol(t)} + \mathcal O(\scp^2)\\
&= \frac{\scp}{4}\ICinv(t)\,a(\pos_t)\,\mltPot'''(\pos_t) + \mathcal O(\scp^2).
\end{align}
For the variational approximation, the analysis is similar but slightly more involved. 
By Taylor expansion and the Leibniz rule, we have  
\begin{align}
    & a(x)\, \partial_x \left( \mltPot(x)-\mltPot^{\rm va}_{\rm eff}(t,x) \right) \\
    & = 
    \sum_{k=0}^5 \sum_{j=0}^k \frac{a^{(j)}(\pos_t) }{j!(k-j)!}  
    \,
    \partial_x^{k-j+1}
    \bigl( \mltPot(\pos_t)-\mltPot^{\rm va}_{\rm eff}(t,\pos_t) \bigr)
    (x-\pos_t)^{k}
    + \mathcal O((x-\pos_t)^6).
\end{align}
%
We now use that 
\begin{align}
    a_1(t) &= \mltPot'(\pos_t) + 
    \tfrac12\mltPot'''(\pos_t)\mean{ (x-\pos_t)^2} + 
    \tfrac{1}{4!} \mltPot^{(5)}(\pos_t)\mean{(x-\pos_t)^4} 
    + \mathcal O(\scp^3),\\
    A_2(t) &= \mltPot''(\pos_t) + 
    \tfrac12\mltPot^{(4)}(\pos_t)\mean{(x-\pos_t)^2} 
    %+     \tfrac{1}{4!} \mltPot^{(6)}(\pos_t)\mean{(x-\pos_t)^4} 
    + \mathcal O(\scp^2).
\end{align}
Then, we average and keep the even powers in $x-\pos_t$, to obtain 
\begin{align}
\mean{ a\,\partial_x\bigl(\mltPot-\mltPot_{\rm eff}^{\rm var}(t)\bigr)}
&= a'(\pos_t) \mltPot^{(4)}(\pos_t)
\Bigl( \tfrac{1}{3!} \mean{(x-\pos_t)^4}- \tfrac12 \mean{(x-\pos_t)^2}^2\Bigr) \\
& \quad + \tfrac14 a''(\pos_t) \mltPot'''(\pos_t)
 \Bigl( \mean{(x-\pos_t)^4} - \mean{(x-\pos_t)^2}^2 \Bigr) +
\mathcal O(\scp^3)\\
&= \tfrac{1}{8} \, a''(\pos_t) \mltPot'''(\pos_t) \,\scp^2 \IC(t)^{-2} + 
\mathcal O(\scp^3).
\end{align}
Here, the last identity follows again from \eqref{eq:moments}.
\end{proof}




==> old-stuff/ausblick.tex <==
\bigskip



{\bf Material fuer den Ausblick -- das muss man nicht bringen}
For instance, given the enormous interest in quantum information processing
schemes via arrays of Penning traps (see, e.q.~\cite{JaiS2024}), our above example 
of simulating the quantum dynamics of a charged particle in a single trap 
can serve as a starting point for more complex simulations that involve
multiple particles and/or multiple traps. Similarly, our computational
framework can also be applied to other trapping schemes such as Paul 
traps, see e.g.~\cite{MatY2021}. 

\bigskip



{\bf Material fuer Anhang}\\ 
In order to construct an analytical reference solution for 
Eq.~\eqref{eq:TDSE-EM} or, equivalently, Eq.~\eqref{eq:TDSE-no-units}, 
it is useful to introduce the operators
\begin{align}
	\label{eq:annihilation_cartesian}
	\hat{a}_x & = \frac{1}{\sqrt{2 \hbar}} \left(
	\sqrt{\frac{m \Omega}{2}} \, x + i \sqrt{\frac{2}{m \Omega}} \, \hat{p}_x
	\right), \\
	\hat{a}_y & = \frac{1}{\sqrt{2 \hbar}} \left(
	\sqrt{\frac{m \Omega}{2}} \, y + i \sqrt{\frac{2}{m \Omega}} \, \hat{p}_y
	\right), \\	              
	\hat{a}_z & = \frac{1}{\sqrt{2 \hbar}} \left(
	\sqrt{m \axialFreq} \, z + i \sqrt{\frac{1}{m \axialFreq}} \, \hat{p}_z
	\right), 	 	              
\end{align}
and to transform $\hat{a}_x$ and $\hat{a}_y$ according to. 
\begin{align}
	\label{eq:annihilation_pm}
	\begin{pmatrix}
		\hat{a}_+ \\
		\hat{a}_-
	\end{pmatrix}
	= \frac{1}{\sqrt{2}} \begin{pmatrix}
		1 & i \\
		i & 1
	\end{pmatrix}
	\begin{pmatrix}
		\hat{a}_x \\
		\hat{a}_y
	\end{pmatrix}.
\end{align}
The only non-vanishing commutators of these operatprs are 
\begin{align}
   \left[\hat{a}_+,\hat{a}_+^\dagger \right] 
   =
   \left[\hat{a}_-,\hat{a}_-^\dagger \right]
   =
   \Big[\hat{a}_z,\hat{a}_z^\dagger \Big] = 1.
\end{align}
This allows us to rewrite the Hamilton operator on the r.h.s. of Eq.~\eqref{eq:TDSE-EM} as (see also Ref.~\cite{CriGV2018})
\begin{align}
	\label{eq:harmonic-oscillators}
   \hat{H} 
   = 
	\hbar \omega_+ \left( \hat{a}_+^\dagger \hat{a}_+ + \frac{1}{2}\right)
	-
	\hbar \omega_- \left( \hat{a}_-^\dagger \hat{a}_- + \frac{1}{2}\right)
	+
	\hbar \axialFreq \left( \hat{a}_z^\dagger \hat{a}_z + \frac{1}{2}\right).
\end{align}
The eigenvalues of this Hamilton operator are 
$\hbar \omega_+ n_+ - \hbar \omega_- n_- + 	\hbar \axialFreq n_z + E_0 $, where
$n_+,n_-,n_z \in \mathbb{N}_0$ and $E_0 = \hbar (\Omega + \axialFreq)/2$. 
The normalized eigenfunction corresponding to the eigenvalue $E_0$ then 
becomes
\begin{align}
    \phi_0(x,y,z) 
	= 
	\left(
       \frac{1}{\textcolor{KITred}{4}\pi^3}
       \frac{m^3}{\hbar^3} \Omega^2 \axialFreq
	\right)^{1/4}
	\exp \left( 
	      - \frac{1}{2}\left( \frac{x^2+y^2}{\lambda_0^2} 
	                          + 
	                          \frac{z^2}{\lambda_z^2} \right)
	      \right),
\end{align}
where we have introduced $\lambda_0 = \sqrt{2\hbar/m\Omega}$ and
$\lambda_z = \sqrt{\hbar/m\axialFreq}$.

Analogous to Ref.~\cite{FerV09}, we can construct from this eigenstate 
coherent states by successively applying the displacement operators
$\hat{D}_+(\alpha_+)$, $\hat{D}_-(\alpha_-)$, and $\hat{D}_z(\alpha_z)$
of the individual harmonic oscillators in the Hamilton operator
\eqref{eq:harmonic-oscillators} .
These displacement operators are defined via
\begin{align}
	\label{eq:displacement}
	\hat{D}(\alpha)
	=
	e^{\alpha \hat{a}^\dagger-\alpha^* \hat{a}}
	=
	e^{-\frac{1}{2} \vert \alpha \vert^2}
	e^{\alpha \hat{a}^\dagger}
	e^{-\alpha^* \hat{a}}
\end{align}
Using the Heisenberg equation of motion,, we obtain for the complex
amplitudes
\begin{align}
	\label{rq:alpha-plus}
	\alpha_+ (t) & = \left(c_+(t) + i s_+(t) \right) = \alpha_+(0) \, e^{-i\omega_+ t}, \\
	\label{rq:alpha-minus}
	\alpha_- (t) & = \left(c_-(t) + i s_-(t) \right) = \alpha_-(0) \, e^{i\omega_- t}, \\
	\label{rq:alpha-z}
	\alpha_z (t) & = \left(c_z(t) + i s_z(t) \right) = \alpha_z(0) \, e^{-i\axialFreq t}, 
\end{align}
and via the expectation values of the position and veloctity operatprs, 
these amplitudes are directly connected to the classical trajectories
via
\begin{align}
	\label{eq:classical-trajectory}
	\begin{pmatrix}
		x_c(t) \\
		y_c(t) \\
		z_c(t)
	\end{pmatrix}
	& =
	\begin{pmatrix}
		\lambda_0 \left( c_+(t) + s_-(t) \right) \\
		\lambda_0 \left( s_+(t) + c_-(t) \right) \\
		\sqrt{2} \lambda_z c_z(t)
	\end{pmatrix}, \\
	\label{eq:classical-velocity}
	\begin{pmatrix}
		\textcolor{KITred}{p}_x(t) \\
		\textcolor{KITred}{p}_y(t) \\
		\textcolor{KITred}{p}_z(t)
	\end{pmatrix}
	& =
	\frac{\hbar}{m}
	\begin{pmatrix}
		\left( s_+(t) - c_-(t) \right)/\lambda_0  \\
		\left( s_-(t) - c_+(t) \right)/\lambda_0 \\
		\sqrt{2} s_z(t)/\lambda_z
	\end{pmatrix}.
\end{align}
As a result, we obtain the time evolution of the coherent state wave function
in terms of the classical trajectory as (see also Ref.~\cite{BiaB24})
\begin{align}
	\label{eq:coherent-state}
	\psi_c(\vec{r},t)
	& =
	e^{i \left( c_+(t)c_-(t) - s_+(t)s_-(t) - c_z(t)s_z(t) \right)} \,
	e^{i m \left( \textcolor{KITred}{p}_x(t)x + \textcolor{KITred}{p}_y(t)y + \textcolor{KITred}{p}_z(t) \right) / \hbar} \cdot 
	\nonumber \\
	& \phantom{=}
	\cdot \phi_0(x-x_c(t), y-y_c(t), z-z_c(t))).
\end{align}


==> old-stuff/old-stuff-section3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FROM SECTION~2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Equations in terms of $V$}
For magnetic Schr\"odinger operators in Coulomb gauge, it is convenient to write
\begin{equation}\label{eq:hamilton_splitted}
    H(t) = -\frac{\scp^2}{2}\Delta_x + \ii\scp \mgPot(t,x)\cdot\nabla_x + \mPot(t,x),\quad \mPot(t,x) = \frac12|\mgPot(t,x)|^2 + \mltPot(t,x) 
\end{equation}
Following \cite[Section3.1]{BurDHL24}, the variational equations of motion for the parameters of the \GWP can then be written as 
\begin{subequations}\label{eq:hageqmo}
		\begin{align+}
			\dot{\pos} &= \mom - \langle \mgPot\rangle_{\vsol} \label{eq:ham-q}\\
			\dot{\mom} &=  \langle J_{\mgPot}^\top \rangle_{\vsol} \mom - \langle \nabla \mPot \rangle_{\vsol} + \scp\remain{\mom}
            \label{eq:ham-p}\\
         	\dot{\fcQ} &= \fcP - \l\langle J_{\mgPot}\r\rangle_{\vsol} \fcQ,
            \label{eq:eqmo_Q}\\
		    \dot{\fcP} &= \langle J_{\mgPot}^\top\rangle_{\vsol} \fcP + 
		\left( \l\langle  D^2_{\mgPot,\mom}\r\rangle_{\vsol}  -
		\bigl\langle \nabla^2 \mPot \bigr\rangle_{\vsol} + \scp\remain{\fcP}\right)\fcQ
        \label{eq:eqmo_P}
        \\
			\dot{\pha} &= \tfrac{1}{2} |\mom|^2  - \langle \mPot\rangle_{\vsol} + \scp\remain{\pha}
		\end{align+}
		%
		%with initial data $(\pos(0),\mom(0), \fcQ(0), \fcP(0), \pha(0)) = (\pos_0, \mom_0, \fcQ_0, \fcP_0, \pha_0)$.
\end{subequations}
with remainder terms of the form
\begin{subequations} \label{eq:remain-all}
\begin{align+}
\remain{\mom} &= \frac{1}{2}\l\langle\nabla\tracemat\r\rangle_{\vsol},\quad 
\remain{\fcP} = \frac{1}{2} \bigl\langle \nabla^2 \tracemat\bigr\rangle_{\vsol},  \\
%\remain{\pha} &=  %\frac{1}{2} \bigl\langle  \tracemat\bigr\rangle_{\vsol}  
                  %\frac{\ii}{2} \tr (\wm)
                  %+ \frac{1}{4}\tr\bigl(\ICinv \bigl\langle \nabla^2 \mPot\bigr\rangle_u\bigr)\label{eq:eqmo_pha}% \\
			%&\quad 
			%- \frac{1}{4}\tr\Bigl( \ICinv\bigl(\frac{\scp}{2} \bigl\langle \nabla^2 \tracemat)\bigr\rangle_{\vsol} 
			%+ \langle  D^2_{\mgPot,\mom}\rangle_{\vsol}\bigr)\Bigr). \nonumber \\
            \remain{\pha} &=  %\frac{1}{2} \bigl\langle  \tracemat\bigr\rangle_{\vsol}  
                  \frac{1}{4} \tr \Bigl( 2\ii\wm
                  + \ICinv \bigl(\bigl\langle \nabla^2 \mPot\bigr\rangle_u\label{eq:eqmo_pha}% \\
			%&\quad 
			- \frac{\scp}{2} \bigl\langle \nabla^2 \tracemat)\bigr\rangle_{\vsol} 
			  - \langle  D^2_{\mgPot,\mom}\rangle_{\vsol}\bigr)\Bigr),
\end{align+}
using the short hand notation \textcolor{red}{Achtung: nur rote Identit\"at stimmt}
\begin{align+}  \label{eq:tracemat}
    \tracemat = \tr\!\l(J_{\mgPot} \RC \ICinv \r) 
    \textcolor{red}{=\tr\!\l(J_{\mgPot}^\top \ICinv \RC \r)}
    = \tr\!\l(J_{\mgPot}^\top \RC \ICinv \r).
\end{align+}
\end{subequations}
%
In \cite[Corollary 3.3]{BurDHL24}, it was shown that $\fcQ(t)$ and $\fcP(t)$ are symplectic for all times $t \in\bbR$
if the initial matrices $\fcQ_0$ and $\fcP_0$ are symplectic.

\textcolor{red}{Now we turn $d=3$ using $\times$, don't we?}
We introduce the averaged magnetic momentum, its linearization and the field
\begin{subequations}\label{eq:aux-variable}
    \begin{align}
        \vel &\da \mom - \mean{\mgPot}, \label{eq:aux-variable-v}\\
        \fcVel &\da \fcP - \mean{ \jacobian{\mgPot}}\fcQ. \label{eq:aux-variable-Y}\\
        \mgField &= \mean{\curl\mgPot}.   
    \end{align}
\end{subequations}
Then, we transform the \ODEs~\eqref{eq:hageqmo} in such a way that they structurally mimic the classical equations 
for a charged particle, that is, 
\begin{equation}\label{eq:classical-EM-system}
        \dot{\pos} = \vel, \qquad
        \dot{\vel} = \vel\times \mgField + \elField.
\end{equation}

%we can apply the Boris algorithm. 



% In the following Lemma we derive a transformation of~\eqref{eq:hageqmo} with \eqref{eq:remain-all} into a representation similar to~\eqref{eq:classical-EM-system}.

\begin{lemma}\label{Lemma:euler-lagrange-q-v}
    With the averaged magnetic momenta \(\vel\) defined in~\eqref{eq:aux-variable-v}, the ordinary differential equations~\eqref{eq:ham-q} and~\eqref{eq:ham-p} can be transformed as
    \begin{subequations}\label{eq:euler-lagrange-q-v-old}
        \begin{align+}
            \dot{\pos} &= \vel, \label{eq:eul-lag-q-old} \\
            \dot{\vel} &= \vel\times\mean{\mgField} + \auxPot, \label{eq:eul-lag-v-old}
        \end{align+}
    \end{subequations}

     
    
    \begin{align+}\label{eq:q-v-potential}
        \auxPot 
        &= %\frac{\scp}{2}\mean{\nabla\tr\left(\jacobian{\mgPot}^\top\ReC\ImCinv\right)} 
        \mean{\jacobian{\mgPot}^\top}\mean{\mgPot} 
        - \mean{\nabla \mPot}  
        - \mean{\pt\mgPot} 
        + \scp \remain{\elField},%\frac{\scp}{2}\mean{\auxDervMgPot{\someMatrix}} ,
    \end{align+}
    and remainder 
    \[
    \remain{\elField} = \remain{\mom} +  \frac{1}{2}\mean{\auxDervMgPot{\someMatrix}},
    \]
    where 
    \begin{subequations} \label{eq:euler-lagrange-all}
    \begin{equation}\label{eq:trhessianMgPot_i}
        \left(\auxDervMgPot{\someMatrix}\right)_i 
        \da 
        % \sum\limits_{\ell, k = 1}^d\ptl_k\ptl_\ell \mgPot_i(x)d_{\ell k} 
        % = 
        \tr\left(\hessian{\mgPot_i}\someMatrix\right)
        \quad\text{with}\quad
    % \end{equation}
    % with
    % \begin{equation} \label{eq:defD}
        \someMatrix = (\mean{\jacobian{\mgPot}} - \ReC)\ImCinv .
    \end{equation}
    \end{subequations}
\end{lemma}
\begin{proof}
    First, we differentiate~\eqref{eq:aux-variable-v} and insert~\eqref{eq:ham-p}
    \begin{align}
        \dot{\vel} 
        &= \dot{\mom} 
        - \mean{\pt\mgPot} 
        - \int_{\Rd}\mgPot(t, x)\pt\abs{\vsol(t, x)}^2\dx \\
        &= \mean{\jacobian{\mgPot}}^T\mom 
        - \mean{\pt\mgPot} 
        + \frac{\scp}{2}\mean{\nabla\tracemat} 
        - \mean{\nabla\mPot} %\\
        %&\quad
        - \int_{\Rd}\mgPot(t, x)\pt\abs{\vsol(t, x)}^2\dx \label{eq:derv_v}
    \end{align}
    % For the derivative \(\pt\abs{\vsol(t, x)}^2\) we get
    % \begin{align}
    %     &\!\!\!\pt\abs{\vsol(t, x)}^2 \nonumber\\
    %     &\!\!\!= \abs{\vsol(t, x)}^2\bigg(\frac{2}{\scp}(x-\pos(t))^T\ImC(t)\vel(t) - \tr(\ReC)\nonumber\\
    %     &\!\!\!\quad\qquad\qquad 
    %     - \frac{1}{\scp}(x-\pos(t))^T(\mean{ \jacobian{\mgPot}}^T\ImC + \ImC\mean{ \jacobian{\mgPot}} 
    %     - \im(\wm^2))(x-\pos(t))\bigg),
    % \end{align} 
    % leading to
    % \begin{align}
    %     \int_{\Rd}\mgPot(t, x)\pt\abs{\vsol(t, x)}^2\dx &= I_1 - I_2 + I_3 - \mean{\mgPot}\tr(\ReC)
    % \end{align}
    % with
    % \begin{align}
    %     I_1 
    %     &\da \intRd\mgPot(x)\frac{2}{\scp}(x - \pos)^T\ImC\vel\abs{\vsol(x)}^2\dx, \\
    %     I_2 
    %     &\da \frac{2}{\scp}\intRd \mgPot(x)(x-\pos)^T\mean{ \jacobian{\mgPot}}^T\ImC(x-\pos)\abs{\vsol(x)}^2\dx, \\
    %     I_3
    %     &\da \frac{1}{\scp}\intRd \mgPot(x)(x-\pos)^T\im(\wm^2)(x-\pos)\abs{\vsol(x)}^2\dx.
    % \end{align}
    % where we ignore the time dependence \(t\) in the further course. 
    %
    % For the integral \(I_1\) we get with
    % \begin{align}\label{eq:gradAbsGWP}
    %     \nabla\abs{\vsol(x)}^2 = -\frac{2}{\scp}\ImC(x-\pos)\abs{\vsol(x)}^2
    % \end{align}
    % and partial integration
    % \begin{align}
    %     I_1 = \mean{\jacobian{\mgPot}}\vel.
    % \end{align}
    % We eliminate the factor $\scp^{-1}$ in \(I_2\) with~\eqref{eq:gradAbsGWP} and Lemma~\ref{aux:lemma:integral-1} leading to
    % \begin{align}
    %     I_2
    %     = \frac{\scp}{2}\mean{ \auxDervMgPot{\mean{ \jacobian{\mgPot}}\ImCinv}} 
    %     + \mean{\mgPot}\tr\mean{ \jacobian{\mgPot}^T}
    %     = \frac{\scp}{2}\mean{ \auxDervMgPot{\mean{ \jacobian{\mgPot}}\ImCinv}} \ ,
    % \end{align}
    % where we have used \(\Div\mgPot = 0\) in the last equality. Analogously we transform \(I_3\) using
    % \begin{equation}
    %     \im(\wm^2) = \ReC\ImC + \ImC\ReC \quad\text{and}\quad \tr(\ImC\ReC\ImCinv) = \tr \ReC
    % \end{equation}
    % into
    % \begin{align}
    %     I_3
    %     &= \frac{\scp}{4}\mean{ \auxDervMgPot{\ReC\ImCinv}} 
    %     + \frac{\scp}{4}\mean{ \auxDervMgPot{\ImCinv\ReC}} 
    %     + \mean{\mgPot}\tr \ReC \ .
    % \end{align}
    By using Lemma~\ref{Lemma:intPotdtAbsGWP}, for each component of \(\mgPot\) we get
    \begin{align}
        \int_{\Rd}\mgPot(t, x)\pt\abs{\vsol(t, x)}^2\dx 
        &= 
        \mean{\jacobian{\mgPot}}\vel 
        - 
        \frac{\scp}{2}\mean{\auxDervMgPot{\someMatrix}} , \label{eq:intMgPotdtAbsGWP}
    \end{align}
    with \(\auxDervMgPot{\someMatrix}\) defined in~\eqref{eq:trhessianMgPot_i}.
    
    Eliminating the \(\mom\) component in~\eqref{eq:derv_v} by~\eqref{eq:aux-variable-v} and inserting~\eqref{eq:intMgPotdtAbsGWP} yields
    \begin{align}
        \dot{\vel} 
        &= % \mean{\jacobian{\mgPot}}^T\vel         - \mean{\jacobian{\mgPot}}\vel
        \vel\times\mean{\mgField}
        + \mean{\jacobian{\mgPot}}^T\mean{\mgPot}
        - \mean{\pt\mgPot} %\\
        %&\quad 
        + \frac{\scp}{2}\mean{\nabla\tracemat} 
        - \mean{\nabla\mPot} 
        + \frac{\scp}{2}\mean{\auxDervMgPot{\someMatrix}} ,
    \end{align}
    where we have used the identity
    \begin{equation}\label{eq:jacobian-to-cross}
        \mean{\left(\jacobian{\mgPot}^\top - \jacobian{\mgPot}\right)v} 
        = \mean{\vel\times\mgField} 
        = \vel\times\mean{\mgField}
    \end{equation}
    in the last step.
\end{proof}

Now we transform the equations of the Hagedorn factorization~\eqref{eq:eqmo_Q} and~\eqref{eq:eqmo_P} to get a similar representation as the classical equations of motion~\eqref{eq:classical-EM-system}. 
\begin{lemma}\label{Lemma:euler-lagrange-Q-Y}
    With the matrix $\fcVel$ defined in~\eqref{eq:aux-variable-Y}, the differential equations \eqref{eq:eqmo_Q} and \eqref{eq:eqmo_P} can be transformed as
    \begin{subequations}\label{eq:euler-lagrange-Q-Y}
        \begin{align+}
            \dot{\fcQ} &= \fcVel, \label{eq:euler-lagrange-Q} \\
            \dot{\fcVel} &= \fcVel\times\mean{\mgField} + \auxauxPot\fcQ, \label{eq:euler-lagrange-Y}
        \end{align+}
    \end{subequations}
    where $\fcVel\times\mean{\mgField} := (\upsilon_1\times \mean{\mgField},\ldots,\upsilon_d\times\mean{\mgField})$ is determined by the cross product of the column vectors $\upsilon_1,\ldots,\upsilon_d$ of $\fcVel$ with $\mean{\mgField}$ and 
    \begin{align+}\label{eq:Q-Y-potential}
        \auxauxPot 
        &= 
        \mean{ \jacobian{\mgPot}^T}\mean{ \jacobian{\mgPot}} 
        + \mean{ \DtwoAvec{\vel + \mean{\mgPot}}} 
        - \mean{ \jacobian{\mgPot_{\ptl, \vel}}} 
        - \mean{\nabla^2\mPot}
        - \mean{\pt\jacobian{\mgPot}} 
        + \scp\remain{S},
    \end{align+}
    where $\jacobian{\auxDervMgPot{\someMatrix}}$ is the Jacobian of $\auxDervMgPot{\someMatrix}$ defined in~\eqref{eq:euler-lagrange-all} 
    % with 
    % \begin{equation}
    %     \someMatrix = (\mean{\jacobian{\mgPot}} - \ReC)\ImCinv
    % \end{equation}
    and $\jacobian{\Aptlv}$ is the Jacobian of
    \begin{equation}
        \Aptlv(x) \da 
        % \begin{pmatrix}
        %     \sum_{i=1}^d\ptl_i\mgPot_1(x)v_i \\
        %     \sum_{i=1}^d\ptl_i\mgPot_2(x)v_i \\
        %     \sum_{i=1}^d\ptl_i\mgPot_3(x)v_i     
        % \end{pmatrix} 
        % = 
        \jacobian{\mgPot}(x)v 
    \end{equation}
    and remainder
    \[
    \remain{S} = \remain{P} + \tfrac12 \mean{\jacobian{\auxDervMgPot{\someMatrix}}} .
    \]
\end{lemma}
\begin{proof}
    We start by differentiating~\eqref{eq:aux-variable-Y} as
    \begin{equation}\label{eq:derv_R}
        \dot{\fcVel} = \dot{\fcP} - \left(\totalDervt\mean{ \jacobian{\mgPot}}\right)\fcQ - \mean{ \jacobian{\mgPot}}\fcVel.
    \end{equation}
    Inserting~\eqref{eq:eqmo_P} into~\eqref{eq:derv_R} and using~\eqref{eq:aux-variable-Y} as well as~\eqref{eq:jacobian-to-cross} column-wise in \(\fcVel\) results in
    \begin{align}
        \dot{\fcVel} 
        &= \fcVel\times\mean{\mgField} 
        + \mean{ \jacobian{\mgPot}^T}\mean{ \jacobian{\mgPot}}\fcQ 
        + \frac{\scp}{2}\mean{ \nabla^2\tracemat}\fcQ \nonumber\\
        &\quad\,+ \mean{\DtwoAvec{p}}\fcQ 
        - \mean{\nabla^2\mPot}\fcQ 
        - \left(\totalDervt\mean{ \jacobian{\mgPot}}\right)\fcQ \ .\label{Ch5:eq:ODE_R}
    \end{align}
    Next we differentiate
    \begin{equation}\label{eq:mean_dtJ_A}
        \totalDervt\mean{\jacobian{\mgPot}} = \mean{\pt\jacobian{\mgPot}} + \intRd\jacobian{\mgPot}(x)\pt\abs{\vsol(x)}^2\dx
    \end{equation}
    and with Lemma~\ref{Lemma:intPotdtAbsGWP} used on each component of \(\jacobian{\mgPot}\) we get
    \begin{align}
        \intRd \jacobian{\mgPot}(x)\pt\abs{\vsol(x)}^2\dx 
        &= 
        \mean{ \jacobian{\Aptlv}} 
        - 
        \frac{\scp}{2}\mean{ \jacobian{\auxDervMgPot{\someMatrix}}} \ . \label{eq:J_A_timeDervAbsGWP_final}
    \end{align}
    Inserting~\eqref{eq:J_A_timeDervAbsGWP_final} into~\eqref{eq:mean_dtJ_A} and~\eqref{eq:mean_dtJ_A} into~\eqref{Ch5:eq:ODE_R} proves the statement.
\end{proof}



